GeoRefine: Self-Supervised Online Depth Refinement for Accurate Dense Mapping

We present a robust and accurate depth refinement system, named GeoRefine, for geometrically-consistent dense mapping from monocular sequences. GeoRefine consists of three modules: a hybrid SLAM module using learning-based priors, an online depth refinement module leveraging self-supervision, and a global mapping module via TSDF fusion. The proposed system is online by design and achieves great robustness and accuracy via: (i) a robustified hybrid SLAM that incorporates learning-based optical flow and/or depth; (ii) self-supervised losses that leverage SLAM outputs and enforce long-term geometric consistency; (iii) careful system design that avoids degenerate cases in online depth refinement. We extensively evaluate GeoRefine on multiple public datasets and reach as low as $5\%$ absolute relative depth errors.

==> figures/euroc_fusion.tex <==
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.4\textwidth]{GeoRefine/images/euroc_fusion.png}
\end{center}
\vspace{-0.5cm}
\caption{Global reconstruction of the EuRoC Vicon room using the refined depth maps by GeoRefine.}
\label{fig:euroc_fusion}
\vspace{-0.4cm}
\end{figure}

==> figures/euroc_qualitative.tex <==
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.9\textwidth]{images/euroc_compare.png}
\end{center}
\vspace{-0.4cm}
\caption{Additional EuRoC Qualitative Results. Refined depth from our method is able to eliminate many artifacts and erroneous predictions compared to Monodepth2.}
\label{fig:euroc_qualitative}
\end{figure}

==> figures/kitti_qualitative.tex <==
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.95\textwidth]{images/kitti_compare.png}
\end{center}
\vspace{-0.5cm}
\caption{KITTI Eigen Split Results. We find that our method is able to better infer foreground-background details than Monodepth2.}
\label{fig:kitti_qualitative}
\end{figure}

==> figures/kitti_results.tex <==
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.48\textwidth]{images/kitti_results.PNG}
\end{center}
\caption{The absolute relative errors of randomly sampled sequences from the KITTI eigen test set. Our method achieves consistent improvements compared to Monodepth2.}
\label{fig:kitti_results}
\end{figure}

==> figures/trajectory_euroc.tex <==
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.36\textwidth]{images/ResultsComparison.png}
\end{center}
\caption{Comparison of camera trajectories by two versions of CNN SLAM with and without using scale self-correction on EuRoC Sequence V2\_01. The trajectory with scale correction aligns better with the groundtruth than the one without scale correction.}
\label{fig:traj_euroc}
\end{figure}

==> figures/tum_fusion.tex <==
\begin{figure*}[!t]
\begin{center}
\includegraphics[width=0.45\textwidth]{GeoRefine/images/tum00.png}
\end{center}
\vspace{-0.5cm}
\caption{Global reconstruction on TUM-RGBD using the refined depth maps by GeoRefine.}
\label{fig:tum_fusion}
\vspace{-0.4cm}
\end{figure*}

==> tables/euroc_mono_eval_all_tab.tex <==
\begin{table}[!t]
    \centering
    \caption{Quantitative depth evaluation on the EuRoC dataset in the monocular mode. Per-frame scale alignment with the groundtruth depth is performed as in Monodepth2~\cite{godard2019digging}.}
    \label{tab:euroc_all_eval_mono}
    % \vspace{-0.2cm}
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{Method} & 
    \multicolumn{3}{c|}{Error Metric} &  \multicolumn{3}{c|}{Accuracy Metric} \\
    % \hline
    \cline{2-7}
    ~ & MAE & Abs Rel & RMSE  & $\delta_1$ & $\delta_2$ & $\delta_3$ \\
    \hline
    \multicolumn{7}{c}{V1\_01} \\
    \hline
    DPT~\cite{ranftl2021vision} &   0.387  &   0.140  &  0.484   &    0.832  &   0.966  &   0.990   \\
    Ours-DPT-Mono &   {\bf 0.168}  &   {\bf 0.058}  &   {\bf 0.255}  &  {\bf 0.969}  &  {\bf 0.991}  &  {\bf 0.996}\\
    \hline
    \multicolumn{7}{c}{V1\_02} \\
    \hline
    DPT~\cite{ranftl2021vision} &   0.320  &   0.119    &   0.412  &  0.882  &   0.981  &   0.995 \\
    Ours-DPT-Mono &   {\bf 0.165}  &  {\bf 0.058}   &   {\bf 0.248}  &  {\bf 0.972}  &   {\bf 0.991}  &  {\bf 0.996} \\
    \hline
    \multicolumn{7}{c}{V1\_03} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.305  &   0.111    &   0.413  &   0.886  &   0.967  &   0.988  \\
    DPT~\cite{ranftl2021vision} &   0.305  &   0.112    &    0.396  &  0.890  &   0.984  &   {\bf 0.997}  \\
    Ours-MD2-Mono &   {\bf 0.181}  &   {\bf 0.069}   &    {\bf 0.266}  & {\bf 0.954}  &   {\bf 0.988}  &   0.995  \\
    Ours-DPT-Mono &   0.202  &   0.074    &    0.297   &   0.949  &   0.976  &   0.984  \\
    \hline
    \multicolumn{7}{c}{V2\_01} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.423  &   0.153    &    0.581  &   0.800  &   0.940  &   0.983\\
    DPT~\cite{ranftl2021vision} &   0.325  &   0.128    &   0.436  &   0.854  &   0.959  &   0.990   \\
    MonoIndoor~\cite{ji2021monoindoor} & - &  0.125 & 0.466 & 0.840 & 0.965 & 0.993 \\
    Ours-MD2-Mono &   0.199  &   0.071    &   0.293  &  0.944  &   0.986  &   0.995 \\
    Ours-DPT-Mono &   {\bf 0.193}  &  {\bf 0.063}  &  {\bf 0.277}  &  {\bf 0.959}  &  {\bf 0.993}  &  {\bf 0.998}  \\
    \hline
    \multicolumn{7}{c}{V2\_02} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.597  &   0.191    &   0.803  &   0.723  &   0.911  &   0.965  \\
    DPT~\cite{ranftl2021vision} &   0.404  &   0.134   &   0.540  & 0.838  &   0.958  &   0.989 \\
    Ours-MD2-Mono &   0.214  &   0.073    &   0.341  &  0.954  &  {\bf 0.985}  &  {\bf 0.993} \\
    Ours-DPT-Mono &   {\bf 0.210}  &   {\bf 0.067}   &   {\bf 0.317}  &  {\bf 0.955}  &   0.982  &   0.991  \\
    \hline
    \multicolumn{7}{c}{V2\_03} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.601  &   0.211    &   0.784  &  0.673  &   0.884  &   0.949 \\
    DPT~\cite{ranftl2021vision} &   0.283  &   0.099   &   0.366  &  0.905  &   0.979  &   0.994 \\
    Ours-MD2-Mono &   {\bf 0.192}  &   {\bf 0.064}    &   {\bf 0.266}  &   {\bf 0.956}  &   {\bf 0.992}  &   {\bf 0.998}  \\
    Ours-DPT-Mono &   0.229  &   0.076 & 0.309   &  0.929  &   0.986  &   0.997 \\
    \hline
    \end{tabular}
    }
    % \vspace{-0.4cm}
\end{table}

==> tables/euroc_stereo_eval_all_tab.tex <==
\begin{table}[!t]
    \centering
    \caption{Quantitative depth evaluation on the EuRoC dataset in the visual-inertial mode. Depth maps are predicted in metric scale, \ie, in meters, and no per-frame scale alignment is performed.}
    \label{tab:euroc_all_eval_vio}
    % \vspace{-0.2cm}
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{Method} & 
    \multicolumn{3}{c|}{Error Metric} &  \multicolumn{3}{c|}{Accuracy Metric} \\
    % \hline
    \cline{2-7}
    ~ & MAE & Abs Rel & RMSE  & $\delta_1$ & $\delta_2$ & $\delta_3$ \\
    \hline
    \multicolumn{7}{c}{V1\_01} \\
    \hline
    DPT~\cite{ranftl2021vision} &   0.501  &   0.174  &  0.598   &  0.709  &   0.966  &   0.994     \\
    CodeMapping~\cite{matsuki2021codemapping} &   0.192   &  -    &   0.381  &   -  &   -  & - \\
    Ours-DPT-VI &   {\bf 0.158}  &   {\bf 0.052}  &  {\bf 0.245}   &  {\bf 0.981}  &   {\bf 0.993}  &   {\bf 0.996}    \\
    \hline
    \multicolumn{7}{c}{V1\_02} \\
    \hline
    DPT~\cite{ranftl2021vision} &   0.496  &   0.182    &  0.586  &  0.712  &   0.970  &   {\bf 0.994} \\
    CodeMapping~\cite{matsuki2021codemapping} &   0.259   &   -   &   0.369  &   -  &   -  & - \\
    Ours-DPT-VI &   {\bf 0.166}  &   {\bf 0.058}   &  {\bf 0.251}  &  {\bf 0.972}  &   {\bf 0.988}  &   {\bf 0.994} \\
    \hline
    \multicolumn{7}{c}{V1\_03} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.360  &   0.132  &   0.464  &  0.815  &   0.945  &   0.986 \\
    DPT~\cite{ranftl2021vision} &   0.499  &   0.185   &   0.581 & 0.700  &   0.945  &   0.994 \\
    CodeMapping~\cite{matsuki2021codemapping} &   0.283   &   -   &   0.407  &   -  &   -  & - \\
    Ours-MD2-VI &   {\bf 0.178}  &   {\bf 0.062}    &   {\bf 0.255}  &  {\bf 0.972}  &   {\bf 0.990}  &   {\bf 0.997} \\
    Ours-DPT-VI &   0.196  &   0.074    &   0.280  & 0.955  &   0.984  &   0.990  \\
    \hline
    \multicolumn{7}{c}{V2\_01} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.490  &   0.181  &   0.648   &   0.730  &   0.920  &   0.972\\
    DPT~\cite{ranftl2021vision} &   0.482  &   0.205    &   0.571  &  0.703  &   0.930  &   0.990  \\
    CodeMapping~\cite{matsuki2021codemapping} &   0.290   &   -   &   0.428  &   -  &   -  & -  \\
    Ours-MD2-VI &   {\bf 0.169}  &   {\bf 0.059}   &  0.265  &  {\bf 0.968}  &   {\bf 0.989}  &   {\bf 0.996} \\
    Ours-DPT-VI &   0.180  &   0.067   &  {\bf 0.263}  &   0.964  &   0.986  &   0.995  \\
    \hline
    \multicolumn{7}{c}{V2\_02} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.769  &   0.233  &   0.963 &   0.562  &   0.816  &   0.937 \\
    DPT~\cite{ranftl2021vision} &   0.601  &   0.191   &    0.727  &  0.699  &   0.908  &   0.981  \\
    CodeMapping~\cite{matsuki2021codemapping} &   0.415   &   -   &   0.655  &   -  &   -  & - \\
    Ours-MD2-VI &   {\bf 0.193}  &   {\bf 0.060}    &   {\bf 0.320}  & {\bf 0.964}  &   {\bf 0.988}  &  {\bf 0.994} \\
    Ours-DPT-VI &   0.213  &   0.069   &   0.324  & 0.956  &   0.980  &   0.989  \\
    \hline
    \multicolumn{7}{c}{V2\_03} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.764  &   0.258   &   0.912   &   0.498  &   0.757  &   0.903 \\
    DPT~\cite{ranftl2021vision} &   0.480  &   0.154   &   0.564  & 0.746  &   0.952  &   0.992 \\
    CodeMapping~\cite{matsuki2021codemapping} &   0.686   &   -   &   0.952  &   -  &   -  & - \\
    Ours-MD2-VI &   0.171  &   0.059   &   0.251  & 0.968  &   0.990  &   0.996 \\
    Ours-DPT-VI &   {\bf 0.159}  &   {\bf 0.055}   &   {\bf 0.220}  & {\bf 0.973}  &  {\bf 0.994}  &  {\bf 0.998} \\
    \hline
    \end{tabular}
    }
    % \vspace{-0.4cm}
\end{table}

==> tables/euroc_stereo_eval_all_tab_small_res.tex <==
\begin{table}[!t]
    \centering
    \caption{Quantitative depth evaluation on the EuRoC dataset under a smaller resolution.}
    \label{tab:euroc_all_eval_vio_small}
    % \vspace{-0.2cm}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{Method} & 
    \multicolumn{3}{c|}{Error Metric} &  \multicolumn{3}{c|}{Accuracy Metric} \\
    % \hline
    \cline{2-7}
    ~ & MAE & Abs Rel & RMSE  & $\delta_1$ & $\delta_2$ & $\delta_3$ \\
    \hline
    \multicolumn{7}{c}{V1\_03} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.279  &   0.103   &   0.362  & 0.896  &   0.983  &   {\bf 0.996} \\
    Ours-MD2-VI &   {\bf 0.173}  &   {\bf 0.062}    &   {\bf 0.256}  &  {\bf 0.968}  &   {\bf 0.989}  &   {\bf 0.996} \\
    \hline
    \multicolumn{7}{c}{V2\_01} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.503  &   0.183  &   0.643   &   0.712  &   0.935  &   0.985\\
    Ours-MD2-VI &   {\bf 0.170}  &   {\bf 0.064}   &  {\bf 0.263}  &  {\bf 0.966}  &   {\bf 0.990}  &   {\bf 0.997} \\
    \hline
    \multicolumn{7}{c}{V2\_02} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.645  &   0.202  &  0.811 &   0.648  &   0.894  &   0.966 \\
    Ours-MD2-VI &   {\bf 0.198}  &   {\bf 0.067}    &   {\bf 0.324}  & {\bf 0.962}  &   {\bf 0.986}  &  {\bf 0.993} \\
    \hline
    \multicolumn{7}{c}{V2\_03} \\
    \hline
    Monodepth2 \cite{godard2019digging} &   0.633  &   0.216   &    0.772    &  0.613  &   0.852  &   0.925 \\
    Ours-MD2-VI &   {\bf 0.182}  &   {\bf 0.062}   &   {\bf 0.259}  & {\bf 0.959}  &   {\bf 0.984}  &   {\bf 0.994} \\
    \hline
    \end{tabular}
    }
\end{table}

==> tables/sup_euroc_vio_keyframes_tab.tex <==
% \begin{table}[!t]
%     \centering
%     \caption{Quantitative depth evaluation for keyframes on EuRoC in the visual-inertial mode. Depth maps are predicted in metric scale, \ie, in meters, and no per-frame scale alignment is performed.}
%     \label{tab:euroc_vio_keyframes_sup}
%     % \vspace{-0.2cm}
%     \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{|l|c|c|c|c|c|c|}
%     \hline
%     \multirow{2}{*}{Method} & 
%     \multicolumn{3}{c|}{Error Metric} &  \multicolumn{3}{c|}{Accuracy Metric} \\
%     % \hline
%     \cline{2-7}
%     ~ & MAE & Abs Rel & RMSE  & $\delta_1$ & $\delta_2$ & $\delta_3$ \\
%     \hline
%     \multicolumn{7}{c}{V1\_01} \\
%     \hline
%     Ours-DPT-VI &    0.154  &   0.051  &  0.239   &  0.982  &   0.993  &  0.996    \\
%     \hline
%     \multicolumn{7}{c}{V1\_02} \\
%     \hline
%     Ours-DPT-VI &    0.164  &   0.057   &  0.247  &  0.974  &   0.989  &   0.995  \\
%     \hline
%     \multicolumn{7}{c}{V1\_03} \\
%     \hline
%     Ours-MD2-VI &   0.184  &   0.063   &   0.262   &   0.971  &   0.991  &   0.997  \\
%     Ours-DPT-VI &   0.201  &   0.071    &   0.287  & 0.953  &   0.984  &   0.991  \\
%     \hline
%     \multicolumn{7}{c}{V2\_01} \\
%     \hline
%     Ours-MD2-VI &  0.148  &   0.051   &   0.230   &   0.975  &   0.995  &   0.998  \\
%     Ours-DPT-VI &   0.149  &   0.051   &  0.218  &   0.979  &   0.996  &   0.999  \\
%     \hline
%     \multicolumn{7}{c}{V2\_02} \\
%     \hline
%     Ours-MD2-VI & 0.191  &   0.057  &   0.313  &   0.966  &   0.990  &   0.996  \\
%     Ours-DPT-VI &  0.205  &   0.064   &   0.313  &  0.960  &   0.984  &   0.992  \\
%     \hline
%     \multicolumn{7}{c}{V2\_03} \\
%     \hline
%     Ours-MD2-VI &   0.171  &   0.059   &   0.251  & 0.968  &   0.990  &   0.996 \\
%     Ours-DPT-VI &   0.159  &   0.055   &   0.221  & 0.974  &   0.995  &   0.998  \\
%     \hline
%     \end{tabular}
%     }
%   % \vspace{-0.4cm}
% \end{table}

\begin{table}[!t]
    \centering
    \caption{Quantitative depth evaluation for keyframes on EuRoC.}
    \label{tab:euroc_vio_keyframes_sup}
    % \vspace{-0.2cm}
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{|l|c|c|c|c||c|c|c|c||c|c|c|c|}
    \hline
    \multirow{2}{*}{Method} & 
    \multicolumn{4}{c||}{Monocular} &  \multicolumn{4}{c||}{Visual-Inertial} &  \multicolumn{4}{c|}{pRGBD} \\
    % \hline
    \cline{2-13}
    ~ & MAE $\downarrow$ & AbsRel $\downarrow$ & RMSE $\downarrow$ & $\delta_1$ $\uparrow$ & MAE $\downarrow$ & AbsRel $\downarrow$ & RMSE $\downarrow$ & $\delta_1$ $\uparrow$ & MAE $\downarrow$ & AbsRel $\downarrow$ & RMSE $\downarrow$ & $\delta_1$ $\uparrow$ \\
    \hline
    \multicolumn{13}{c}{V1\_01} \\
    \hline
    Ours-DPT &   {\bf 0.153}  &   {\bf 0.050}  &   {\bf 0.241}  &  {\bf 0.980}  &  {\bf 0.147}  &   {\bf 0.048}  &  {\bf 0.241}   &  {\bf 0.980} & {\bf 0.151} & {\bf 0.049} & {\bf 0.239} & {\bf 0.982} \\
    \hline
    \multicolumn{13}{c}{V1\_02} \\
    \hline
    Ours-DPT &   {\bf 0.171}  &  {\bf 0.058}   &   {\bf 0.255}  &  {\bf 0.967}  &   {\bf 0.166}  &   {\bf 0.058}   &  {\bf 0.251}  &  {\bf 0.972} & {\bf 0.160} & {\bf 0.056} & {\bf 0.240} & {\bf 0.973} \\
    \hline
    \multicolumn{13}{c}{V1\_03} \\
    \hline
    % Ours-MD2 &   {\bf 0.181}  &   {\bf 0.069}   &    {\bf 0.266}  & {\bf 0.954}  &   {\bf 0.178}  &   {\bf 0.062}    &   {\bf 0.255}  &  {\bf 0.972} & & & & \\
    Ours-DPT &   {\bf 0.202}  &   {\bf 0.074}    &    {\bf 0.297}   &   {\bf 0.949}  &  {\bf 0.188}  &   {\bf 0.067}    &   {\bf 0.278}  & {\bf 0.956} & {\bf 0.190} & {\bf 0.068} & {\bf 0.286} & {\bf 0.949} \\
    \hline
    \multicolumn{13}{c}{V2\_01} \\
    \hline
    % Ours-MD2 &   0.199  &   0.071    &   0.293  &  0.944  &   {\bf 0.169}  &   {\bf 0.059}   &  0.265  &  {\bf 0.968} & & & & \\
    Ours-DPT &   {\bf 0.170}  &  {\bf 0.054}  &  {\bf 0.258}  &  {\bf 0.973}  &  {\bf 0.162}  &   {\bf 0.052}   &  {\bf 0.258}  &   {\bf 0.970} & {\bf 0.181} & {\bf 0.057} & {\bf 0.0269} & {\bf 0.970} \\
    \hline
    \multicolumn{13}{c}{V2\_02} \\
    \hline
    % Ours-MD2 &   0.214  &   0.073    &   0.341  &  0.954  &  {\bf 0.193}  &   {\bf 0.060}    &   {\bf 0.320}  & {\bf 0.964} & & & & \\
    Ours-DPT &   {\bf 0.177}  &   {\bf 0.053}   &   {\bf 0.208}  &  {\bf 0.976}  &  {\bf 0.193}  &   {\bf 0.063}   &   {\bf 0.312}  & {\bf 0.966}  & {\bf 0.167} & {\bf 0.053} & {\bf 0.267} & {\bf 0.976} \\
    \hline
    \multicolumn{13}{c}{V2\_03} \\
    \hline
    % Ours-MD2 &   {\bf 0.192}  &   {\bf 0.064}    &   {\bf 0.266}  &   {\bf 0.956}  &   0.171  &   0.059   &   0.251  & 0.968 & & & & \\
    Ours-DPT &   {\bf 0.163}  &   {\bf 0.053} & {\bf 0.231}   &  {\bf 0.970}  &  {\bf 0.159}  &   {\bf 0.055}   &   {\bf 0.220}  & {\bf 0.973} & {\bf 0.152} & {\bf 0.051} & {\bf 0.214} & {\bf 0.975} \\
    \hline
    \end{tabular}
    }
    %\vspace{-0.4cm}
\end{table}
